Optimal strategies for reject option classifiers

In classification with a reject option, the classifier is allowed in uncertain cases to abstain from prediction. The classical cost-based model of a reject option classifier requires the cost of rejection to be defined explicitly. An alternative bounded-improvement model, avoiding the notion of the reject cost, seeks for a classifier with a guaranteed selective risk and maximal cover. We coin a symmetric definition, the bounded-coverage model, which seeks for a classifier with minimal selective risk and guaranteed coverage. We prove that despite their different formulations the three rejection models lead to the same prediction strategy: a Bayes classifier endowed with a randomized Bayes selection function. We define a notion of a proper uncertainty score as a scalar summary of prediction uncertainty sufficient to construct the randomized Bayes selection function. We propose two algorithms to learn the proper uncertainty score from examples for an arbitrary black-box classifier. We prove that both algorithms provide Fisher consistent estimates of the proper uncertainty score and we demonstrate their efficiency on different prediction problems including classification, ordinal regression and structured output classification.

==> extended_tables.tex <==
\section{Experiments}

\subsection{Classification}

\begin{table}
  \begin{sideways}
  \begin{minipage}{1.4\textwidth}
  \centering
    \begin{tabular}{r|cc|cc|cc|cc|c|}
    & \multicolumn{2}{c|}{LR+PLUGIN} 
    & \multicolumn{2}{c|}{LR+SELE} 
    & \multicolumn{2}{c|}{LR+REG}  
    & \multicolumn{2}{c|}{LR+TCP} &   \\
    & AuRC & R@90 &AuRC & R@90 & AuRC & R@90 & AuRC & R@90& R@100 \\  
    \hline
    AVILA &  27.2$\pm$0.6  &  40.9$\pm$0.5  & {\bf 26.0$\pm$0.4} & {\bf 40.0$\pm$0.3 } & 26.7$\pm$0.7  &  40.1$\pm$0.4  & 26.9$\pm$0.8  &  41.1$\pm$0.3  &  43.7$\pm$0.4\\
    %
    CODRNA &  0.9$\pm$0.0  & {\bf 2.0$\pm$0.0 }& {0.7$\pm$0.0} &  2.0$\pm$0.1  & 0.8$\pm$0.1  &  2.3$\pm$0.1  & 0.8$\pm$0.0  &  2.2$\pm$0.1  &  4.8$\pm$0.1 \\
    %
    COVTYPE & {\bf 16.5$\pm$0.1} &  25.1$\pm$0.2  & 17.6$\pm$0.1  &  25.3$\pm$0.2  & 17.6$\pm$0.1  & {\bf 25.0$\pm$0.1 } & 17.2$\pm$0.1  &  25.5$\pm$0.1  &  27.6$\pm$0.2 \\
    %
    IJCNN &  1.3$\pm$0.0  &  3.8$\pm$0.1  &{\bf 1.0$\pm$0.0} & {\bf 3.7$\pm$0.2 }& 1.2$\pm$0.1  &  4.8$\pm$0.3  & 1.1$\pm$0.1  &  4.7$\pm$0.2  &  7.5$\pm$0.1 \\
    %
    LETTER & 7.4$\pm$0.4  &  18.3$\pm$0.6  &{\bf 6.8$\pm$0.3} &  17.8$\pm$0.8  & 7.7$\pm$0.7  &  17.6$\pm$1.2  & 6.8$\pm$0.4  & {\bf 17.4$\pm$0.8 }&  23.3$\pm$0.6\\
    %
    PENDIGIT & {\bf 0.7$\pm$0.0} & {\bf 1.9$\pm$0.1 } & 1.6$\pm$0.2  &  3.2$\pm$0.5  & 1.9$\pm$0.3  &  3.4$\pm$0.5  & 1.6$\pm$0.5  &  2.8$\pm$0.5  &  5.3$\pm$0.4 \\
    %
    PHISHING &  0.8$\pm$0.1  &  2.9$\pm$0.3  &{\bf 0.7$\pm$0.1} &  2.9$\pm$0.1  & 0.9$\pm$0.3  &  3.1$\pm$0.3  & 0.9$\pm$0.3  & {\bf 2.7$\pm$0.3 }&  6.3$\pm$0.4 \\
    %
    SATTELITE & 3.8$\pm$0.3  & {\bf 11.1$\pm$0.4 } &{\bf 3.8$\pm$0.2} &  11.2$\pm$0.4  & 5.5$\pm$1.0  &  11.2$\pm$0.5  & 4.6$\pm$0.6  &  11.2$\pm$0.4  &  15.1$\pm$0.5 \\
    %
    SENSORLESS &  2.0$\pm$0.1  &  4.9$\pm$0.3  &{\bf 1.9$\pm$0.1} &  4.8$\pm$0.1  & 2.7$\pm$0.1  & {\bf 4.4$\pm$0.4 } & 2.4$\pm$0.2  &  4.6$\pm$0.4  &  8.2$\pm$0.4\\
    %
    SHUTTLE &  0.6$\pm$0.1  &  1.0$\pm$0.1  &{\bf 0.3$\pm$0.1} & {\bf 0.6$\pm$0.2 }& 1.4$\pm$0.5  &  0.7$\pm$0.1  & 0.7$\pm$0.1  &  0.9$\pm$0.2  &  3.4$\pm$0.2 \\
    %
    \hline
    wins & 2        &   3 &   8 &  3    &  0    &  2    &  0& 2  \\
    \end{tabular}
    %%
    %%
   \centering
    \begin{tabular}{r|cc|cc|cc|c}
    \multicolumn{8}{c}{}\\
    & \multicolumn{2}{c|}{SVM+MARGIN} 
    & \multicolumn{2}{c|}{SVM+SELE} 
    & \multicolumn{2}{c|}{SVM+REG}  \\
    & AuRC & R@90 &AuRC & R@90 & AuRC & R@90 & R@100 \\  
    \hline
    AVILA &  31.7$\pm$0.8  &  41.0$\pm$0.7  &{\bf 25.4$\pm$0.7} &  39.8$\pm$0.6  & 26.0$\pm$0.8  & {\bf 39.6$\pm$0.6 } &  43.3$\pm$0.7 \\
    %
    CODRNA &  0.9$\pm$0.1  & {\bf 2.0$\pm$0.1 } &{\bf 0.7$\pm$0.0} &  2.0$\pm$0.1  & 0.8$\pm$0.0  &  2.4$\pm$0.1  &  4.8$\pm$0.1 \\
    %
    COVTYPE & 25.7$\pm$0.8  &  26.8$\pm$0.1  & 17.8$\pm$0.2  &  25.4$\pm$0.1  &{\bf 17.8$\pm$0.1} & {\bf 25.1$\pm$0.1 } &  27.4$\pm$0.1 \\
    %
    IJCNN &  1.4$\pm$0.0  & {\bf 3.7$\pm$0.2 } &{\bf1.0$\pm$0.0} &  3.7$\pm$0.2  & 1.2$\pm$0.1  &  4.7$\pm$0.3  &  7.6$\pm$0.2 \\
    %
    LETTER &  10.2$\pm$0.2  &  19.1$\pm$0.4  &{\bf 6.3$\pm$0.5} &  16.4$\pm$1.0  & 7.2$\pm$0.6  & {\bf 16.1$\pm$0.7 }&  22.1$\pm$0.7 \\
    %
    PENDIGIT &  2.8$\pm$0.4  &  3.9$\pm$0.4  &{\bf 1.6$\pm$0.2} & {\bf 2.6$\pm$0.6 }& 2.1$\pm$0.4  &  3.0$\pm$0.5  &  4.9$\pm$0.6 \\
    %
    PHISHING &  0.8$\pm$0.1  &  3.0$\pm$0.3  &{\bf 0.7$\pm$0.1} & {\bf 2.7$\pm$0.3 }& 0.9$\pm$0.3  & 3.0$\pm$0.4  &  6.4$\pm$0.4 \\
    %
    SATTELITE & 4.8$\pm$0.6  & {\bf 11.4$\pm$0.5 } & {\bf 3.9$\pm$0.2} &  11.5$\pm$0.6  & 6.0$\pm$0.7  &  11.6$\pm$0.8  &  15.4$\pm$0.4\\
    %
    SENSORLESS &  3.7$\pm$0.2  &  6.9$\pm$0.3  &{\bf 1.6$\pm$0.1} &  4.3$\pm$0.3  & 2.4$\pm$0.2  & {\bf 4.2$\pm$0.3 }&  6.9$\pm$0.2 \\
    %
    SHUTTLE & 1.3$\pm$0.5  &  1.5$\pm$0.3  &{\bf 0.2$\pm$0.1} & {\bf 0.6$\pm$0.2 } & 0.9$\pm$0.5  &  0.8$\pm$0.1  &  2.0$\pm$0.1 \\
    %
    \hline
    wins & 0    &   3& 9&  3    &  1&  4       \\
    \end{tabular}
    %
    \caption{Caption tady bude pekny popis tohoto krasneho experimentu, ale jeste nevim co presne sm napisu.}
    \end{minipage}
   \end{sideways}
    \label{tab:my_label}
\end{table}


\begin{figure}
    %
    \begin{tabular}{cc}
        AVILA & CODRNA \\
        \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_avila1.eps} &
        \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_codrna1.eps} \\
        COVTYPE & IJCNN \\
        \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_covtype1.eps}&
        \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_ijcnn1.eps}\\
        LETTER & PENDIGIT  \\
        \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_letter1.eps}&
        \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_pendigit1.eps}\\
       PHISHING & SATTELITE \\
       \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_phishing1.eps}&
        \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_sattelite1.eps} \\
        SENSORLESS & SHUTTLE \\
        \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_sensorless1.eps} &
        \includegraphics[width=0.48\columnwidth]{figs/LR+SVM_shuttle1.eps} 
    \end{tabular}
    %
    \caption{The risk-coverage curves for different selective classifiers evaluated on 10 datasets. X-axis is the coverage and y-axis is the selective risk corresponding to the misclassification error on the non-reject area. The classifier is either LR (left sub-figure) or SVM (right sub-figure). 
    %The curves for baseline selective functions shown in black correspond to the the plug-in conditional risk for LR and to the max-score for SVM. Colored curves correspond to selective functions learned by the proposed algorithm on top of linear features (red), quadratic features (green) and features extracted by multi-layer perceptron (blue). 
    }
    \label{fig:results}
\end{figure}


\subsection{Ordinal Regression}


\begin{table}
  \begin{sideways}
  \begin{minipage}{1.4\textwidth}
  \centering
    \begin{tabular}{r|cc|cc|cc|c}
    \multicolumn{8}{c}{}\\
    & \multicolumn{2}{c|}{SVM+MARGIN} 
    & \multicolumn{2}{c|}{SVM+SELE} 
    & \multicolumn{2}{c|}{SVM+REG}  \\
    & AuRC & R@90 &AuRC & R@90 & AuRC & R@90 & R@100 \\  
    \hline
    ABALONE & 148.1$\pm$9.6  &  152.0$\pm$3.0  &{\bf 119.3$\pm$8.8} &  139.1$\pm$2.5 & 121.2$\pm$5.3  & {\bf 137.8$\pm$0.8 }& 153.9$\pm$2.2\\ 
    %
    BANK & 107.2$\pm$4.3  &  147.7$\pm$4.0  & 98.6$\pm$3.8  &  143.4$\pm$2.5  &{\bf 98.0$\pm$3.4} & {\bf 142.1$\pm$2.2 }&  150.4$\pm$2.9 \\
    %
    BIKESHARE &  159.6$\pm$6.6  &  169.2$\pm$2.8  &{\bf 125.1$\pm$1.2} & {\bf 159.1$\pm$3.1 } & 127.2$\pm$0.6  &  159.9$\pm$3.2  &  169.7$\pm$2.7 \\
    %
    CALIFORNIA &  98.1$\pm$2.8  &  116.9$\pm$1.6  &{\bf 81.9$\pm$1.9} &  111.2$\pm$1.2  & 83.7$\pm$2.5  & {\bf 110.6$\pm$1.3 }&  118.2$\pm$1.5 \\
    %
    CPU&  41.2$\pm$1.0  &  61.1$\pm$2.2  &{\bf 35.7$\pm$2.4} & {\bf 57.4$\pm$2.7 }& 36.5$\pm$2.4  &  57.9$\pm$2.6  &  63.5$\pm$2.7 \\
    %
    CCPP &  46.1$\pm$1.8  &  57.1$\pm$1.9  &{\bf 41.4$\pm$2.2} &  55.1$\pm$1.6  & 41.8$\pm$2.4  & {\bf 54.9$\pm$1.7 }&  58.4$\pm$1.8 \\
    %
    GPU &  143.1$\pm$2.2  &  148.1$\pm$1.8  &{\bf 84.7$\pm$2.2} &  131.0$\pm$2.1  & 85.8$\pm$2.0  & {\bf 130.9$\pm$2.0 }&  148.5$\pm$1.9\\
    %
    METRO &  220.1$\pm$6.5  &  233.1$\pm$1.9  &{\bf 197.2$\pm$2.6} & {\bf 226.0$\pm$1.3 } & 197.7$\pm$3.4  &  226.1$\pm$1.1  &  236.7$\pm$2.7 \\
    %
    SUPERCONDUCT &  97.8$\pm$1.7  &  106.4$\pm$1.1  &{\bf 74.9$\pm$1.4} &  98.0$\pm$0.9  & 77.0$\pm$1.3  & {\bf 97.2$\pm$1.0 }&  106.9$\pm$0.8 \\
    %
    FACEBOOK &  51.1$\pm$0.9  &  97.0$\pm$0.7  & 38.4$\pm$1.4  & {\bf 85.9$\pm$1.3 } &{\bf 37.1$\pm$1.1} &  87.4$\pm$1.2  &  110.9$\pm$0.5 \\
    %
    \hline
    wins &0 &   0&       8  & 4 &  2& 6  &\\
    \end{tabular} 
    \end{minipage}
    \end{sideways}
\end{table}


\begin{figure}
    %
    \begin{tabular}{cccc}
        \multicolumn{2}{c}{ABALONE} & \multicolumn{2}{c}{BANK} \\
        \includegraphics[width=0.23\columnwidth]{figs/SVM_abalone1.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_abalone1_examples.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_bank1.eps}  & 
        \includegraphics[width=0.23\columnwidth]{figs/SVM_bank1_examples.eps}
        \\
        %
        \multicolumn{2}{c}{BIKESHARE} & \multicolumn{2}{c}{CALIFORNIA} \\
        \includegraphics[width=0.23\columnwidth]{figs/SVM_bikeshare1.eps}&
        \includegraphics[width=0.23\columnwidth]{figs/SVM_bikeshare1_examples.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_california1.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_california1_examples.eps} \\
        %
        \multicolumn{2}{c}{CCPP} & \multicolumn{2}{c}{CPU} \\
        \includegraphics[width=0.23\columnwidth]{figs/SVM_ccpp1.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_ccpp1_examples.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_cpu1.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_cpu1_examples.eps}\\
        %
        \multicolumn{2}{c}{FACEBOOK} & \multicolumn{2}{c}{GPU} \\
       \includegraphics[width=0.23\columnwidth]{figs/SVM_facebook1.eps}&
       \includegraphics[width=0.23\columnwidth]{figs/SVM_facebook1_examples.eps}&
        \includegraphics[width=0.23\columnwidth]{figs/SVM_gpu1.eps}  &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_gpu1_examples.eps}   \\
        %
        \multicolumn{2}{c}{METRO} & \multicolumn{2}{c}{SUPERCONDUCT} \\
        \includegraphics[width=0.23\columnwidth]{figs/SVM_metro1.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_metro1_examples.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_superconduct1.eps} &
        \includegraphics[width=0.23\columnwidth]{figs/SVM_superconduct1_examples.eps} 
    \end{tabular}
    %
    \caption{The risk-coverage curves for different selective classifiers evaluated on 10 datasets. X-axis is the coverage and y-axis is the selective risk corresponding to the misclassification error on the non-reject area. The classifier is either LR (left sub-figure) or SVM (right sub-figure). 
    %The curves for baseline selective functions shown in black correspond to the the plug-in conditional risk for LR and to the max-score for SVM. Colored curves correspond to selective functions learned by the proposed algorithm on top of linear features (red), quadratic features (green) and features extracted by multi-layer perceptron (blue). 
    }
    \label{fig:results}
\end{figure}


